Influence-Augmented Online Planning for Complex Environments

How can we plan efficiently in real time to control an agent in a complex environment that may involve many other agents? While existing sample-based planners have enjoyed empirical success in large POMDPs, their performance heavily relies on a fast simulator. However, real-world scenarios are complex in nature and their simulators are often computationally demanding, which severely limits the performance of online planners. In this work, we propose influence-augmented online planning, a principled method to transform a factored simulator of the entire environment into a local simulator that samples only the state variables that are most relevant to the observation and reward of the planning agent and captures the incoming influence from the rest of the environment using machine learning methods. Our main experimental results show that planning on this less accurate but much faster local simulator with POMCP leads to higher real-time planning performance than planning on the simulator that models the entire environment.

==> Makefile <==
NAME=neurips_2020

all: 
	pdflatex $(NAME).tex
	make bib
	pdflatex $(NAME).tex
	pdflatex $(NAME).tex
	make clean
	# pdftk neurips_2020.pdf cat 1-10 output submission.pdf 
	# pdftk neurips_2020.pdf cat 11-13 output supplementary_material.pdf 
bib: 
	if [ -e $(NAME).aux ] ; \
	then \
		echo COMPILE BIBTEX; \
		bibtex $(NAME).aux; \
	else \
		echo NO REFERENCES TO COMPILE; \
	fi;
	
clean:
	rm -f $(NAME).aux $(NAME).bbl $(NAME).log $(NAME).out $(NAME).toc $(NAME).blg $(NAME).dvi $(NAME).ps $(NAME).nav $(NAME).snm $(NAME).vrb $(NAME).fdb_latexmk $(NAME).fls

